AgileRate: Bringing Adaptivity and Robustness to DeFi Lending Markets

Decentralized Finance (DeFi) has revolutionized lending by replacing intermediaries with algorithm-driven liquidity pools. However, existing platforms like Aave and Compound rely on static interest rate curves and collateral requirements that struggle to adapt to rapid market changes, leading to inefficiencies in utilization and increased risks of liquidations. In this work, we propose a dynamic model of the lending market based on evolving demand and supply curves, alongside an adaptive interest rate controller that responds in real-time to shifting market conditions. Using a Recursive Least Squares algorithm, our controller tracks the external market and achieves stable utilization, while also controlling default and liquidation risk. We provide theoretical guarantees on the interest rate convergence and utilization stability of our algorithm. We establish bounds on the system's vulnerability to adversarial manipulation compared to static curves, while quantifying the trade-off between adaptivity and adversarial robustness. We propose two complementary approaches to mitigating adversarial manipulation: an algorithmic method that detects extreme demand and supply fluctuations and a market-based strategy that enhances elasticity, potentially via interest rate derivative markets. Our dynamic curve demand/supply model demonstrates a low best-fit error on Aave data, while our interest rate controller significantly outperforms static curve protocols in maintaining optimal utilization and minimizing liquidations.

==> protocolObjectives.tex <==
\subsection{Protocol Objectives and Evaluation Metrics}

Our main objective is to design a protocol for a borrowing and lending pool. The protocol aims to achieve the following:
(i) Accurately estimate future market risks for different players based on current market conditions and historical data.
(ii) Utilize this estimation, along with information about risk-free market rates, to dynamically adjust the pool's parameters (\rt, \liqthrshN, \colfacN and \liqIncntive) in real-time and in response to market changes. We now make these points explicit by defining the following metrics of protocol performance.

% \color{red}
% define profit var lar and efficiencies

% define baseline over which the efficiency is defined to produce gains
% \color{black}

\paragraph{Economic security} The protocol should not lose any money over long period of time but in fact in our solution we enforce it in every single 

\paragraph{Competitiveness}The difference between the risk-free rate of lending/borrowing in the external markets compared to the effective interest rates of the protocol tells us the protocol \textit{competitiveness}. The main objective of the interest rate policy is to ensure the protocol tracks these external rates as closely as possible.


\paragraph{Profit}


We define the profit of a borrowing position from a lender's perspective as the sum total of all cash flows into the lender's account. This includes interest rate payments and any assets lost to insolvencies.

\paragraph{Value-At-Risk (VaR)} 

VaR is a statistical measure that estimates the minimum potential profit of lending position after time \( T \), given a certain confidence level \( \alpha \) (e.g., 95\% or 99\%). Mathematically, VaR can be defined as:

\[
\text{VaR}_\alpha (T) = - \inf \left\{ x \in \mathbb{R} : P(X < x) \leq 1 - \alpha \right\}
\]

where \( X \) is the profit of the borrow position over the time period \( T \), \( \alpha \) is the confidence level (e.g., 0.95 for 95\% confidence), \( P(X > x) \) is the probability that the profit \( X \) is below the value \( x \).


\paragraph{Liquidations-At-Risk (LaR)} 
LaR is a statistical measure that estimates the maximum liquidation of lending position after time \( T \), given a certain confidence level \( \alpha \) (e.g., 95\% or 99\%). Mathematically, LaR can be defined as:

\[
\text{LaR}_\alpha (T) = - \inf \left\{ x \in \mathbb{R} : P(L > x) \leq 1 - \alpha \right\}
\]

where \( L \) is the total amount of liquidations over time \( T \), \( \alpha \) is the confidence level (e.g., 0.95 for 95\% confidence), \( P(L > x) \) is the probability that the liquidations \( L \) exceeds the value \( x \).



\paragraph{Baseline Protocol}
The baseline protocol follows fixed interest rate curves and selects the one which aligns with the equilibrium equation when considering the current expected default rate, mimicking the approach of established DeFi lending protocols. The interest rate is given by
\begin{align}
    r_{t+1} = \mathcal{I}_{\{U_t \leq U^*\}} b_1 U_t + \mathcal{I}_{\{U_t > U^*\}} (b_1 U^* + b_2 (U_t - U^*))
\end{align}
where $\mathcal{I}_{\{.\}}$ is an indicator function, and $b_1 < b_2$ are fixed slope parameters to encourage borrowers/lenders to stay at the desired utilization.

\paragraph{Risk Efficiency}
Finally, we use the notion of risk efficiency to compare our protocols to a baseline. We say that protocol 1 is more \textit{risk-efficient} than protocol 2 if protocol 1 has a larger profit for the same or less VaR value. We aim to develop a lending protocol that is more risk-efficient than the baseline. The main driver behind setting $LT$ should be to make the protocol more risk-efficient.










==> system-design.tex <==
%\section{Blockchain System Design}

